Substructure in clusters containing wide-angle tailed radio galaxies. I. New redshifts

We present new redshifts and positions for 635 galaxies in nine rich clusters containing Wide-Angle Tailed (WAT) radio galaxies. Combined with existing data, we now have a sample of 18 WAT-containing clusters with more than 10 redshifts. This sample contains a substantial portion of the WAT clusters in the VLA 20 cm survey of Abell clusters, including 75% of WAT clusters in the complete survey (z<=0.09), and 20% of WAT clusters with z>0.09. It is a representative sample which should not contain biases other than selection by radio morphology. We graphically present the new data using histograms and sky maps. A semi-automated procedure is used to search for emission lines in the spectra in order to add and verify galaxy redshifts. We find that the average apparent fraction of emission line galaxies is about 9% in both the clusters and the field. We investigate the magnitude completeness of our redshift surveys with CCD data for a test case, Abell 690. This case indicates that our galaxy target lists are deeper than the detection limit of a typical MX exposure, and they are 82% complete down to R=19.0. The importance of the uniformity of the placement of fibers on targets is posited, and we evaluate this in our datasets. We find some cases of non-uniformities which may influence dynamical analyses. A second paper will use this database to look for correlations between the WAT radio morphology and the cluster's dynamical state.

==> tab1.tex <==
%auto-ignore
% \documentstyle[12pt]{article}
% Copy of watradio1.tex.  This version will be modified to 
% work with "aj_pt4.sty" (AASTEX).

\begin{deluxetable}{lccllcrll}
\tablecaption{\sc Radio Properties of WATs}
\tablehead{
\colhead{Source} & \colhead{Cluster}   & \colhead{Alt.Name} & 
\colhead{z\tablenotemark{1}} & \colhead{r/A$_{C}$\tablenotemark{2}} & 
\colhead{log(P$_{1400}$)\tablenotemark{3}} & 
\colhead{Extent\tablenotemark{4}} & \colhead{Morph.\tablenotemark{5}}    & \colhead{Notes\tablenotemark{6}}
}
\startdata
0043+201  &  A98  & 4C20.04 & 0.1063 & 0.08  & 25.12 &  290 & WAT & Z,I,O \nl
0053+261B & A115  &         & 0.1971 & 0.58  & 25.35 &   85 & WAT? & I \nl
0110+152  & A160  &         & 0.0440 & 0.06 & 24.45  &  430   & TJ & Z,I,O \nl 
0255+058A,B  & A400  &  3C75  & 0.0226 & 0.08   & 24.65 &   330   & TJ\&TJ & I,P \nl
0803-008  & A623  &         & 0.0891  &  0.03    & 25.31 &  150  & WAT? & P \nl
0836+290  & A690  & 4C29.30 & 0.0789 &  0.03  &  25.12 &    510    &  WAT & Z,I,O \nl
1138+060    & A1346 &       & 0.0972  &  0.13  & 24.97 & \nodata  & WAT? &   \\
1159+583  & A1446 & 4C58.23 & 0.1025 &  0.09 & 25.24 &  170   &  WAT & Z,I,P,O \nl
1233+168  & A1569 &            & 0.0784 & 0.18  & 25.23  &  350  & WAT? & P \nl
1306+107  & A1684 & 4C10.35 & 0.0864  & 0.28  & 24.80 &  460  & WAT? & Z,O \nl
1313+073  &  \nodata  &    & 0.0507 &  \nodata  & 25.01  &  300  & WAT  &  Z  \nl 
1433+553  & A1940 & 4C55.29 & 0.1402 & 0.07  & 25.28  &    240  & WAT   & I,P,O \nl
1636+379  & A2214 & 4C37.48 & 0.1609 & 0.23  & 25.55  &    450  & WAT   & Z,P,O \nl
1638+538  & A2220 &  &  0.1103  & 0.09  & 25.21 &  240   & WAT & I \nl
1820+689  & A2304 &  &  0.0881  & 0.03  & 25.11 &  170   & WAT? & P \nl
1919+479  & \nodata & 4C47.51 & 0.1022  &  \nodata  & 25.32 &   1200  & WAT & Z,I,P \nl
2236--176 & A2462 & PKS2236-17 & 0.0742 & 0.06 & 25.22 &   200   & WAT  & Z,P,O \nl
2335+267  & A2634 & 3C465 &  0.0302 & 0.04 & 25.17 &   320   & WAT  &  I,P 
\tablenotetext{1}{The redshift, z, is that of the radio galaxy from 
Owen et al. (1988, 1995).}
\tablenotetext{2}{The ratio of the distance of the radio galaxy from the cluster center to the Abell radius.}
\tablenotetext{3}{The logarithmic radio power is given in Watts Hz$^{-1}$
(H$_0$=75 km s$^{-1}$ Mpc$^{-1}$, and q$_0$=0.0), and is calculated
from flux densities given by Owen et al. (1992, 1993) or in OOE. }
\tablenotetext{4}{The maximum, projected, linear size of the source 
(usually between ends of the tails) given in kpc. }
\tablenotetext{5}{These morphologies are suggested by Owen from the 20 cm survey
(Owen, private communication). }
\tablenotetext{6}{ Z: New redshifts presented in this paper.}
\tablenotetext{~}{ I: Observed with {\it Einstein} IPC.}
\tablenotetext{~}{ P: Observed with {\em ROSAT} PSPC.}
\tablenotetext{~}{ O: High resolution radio data in O'Donaghue et al (1990, OOE).  }
\enddata
\end{deluxetable}



==> tab2.tex <==
%auto-ignore
% sub2dtab.tex
% 6/4/96 Follow the sample tables in AASTEX.  For use with the
% style "aj_pt4.sty", and the master file "tables.tex".

\begin{deluxetable}{llccc}
\tablecaption{\sc Log of MX Observing Runs} 
\tablehead{
\colhead{Year}   & \colhead{Date}        & \colhead{Clusters Observed} & 
\colhead{Conditions}     & \colhead{CCD} 
}
\startdata
1991  & Mar 12-13  & A690 c1313+073   & good      & TI 800  \nl
1991  & Dec 29-30  & \nodata          & poor - humid & TI 800  \nl
1991  & Dec 31     & A160 A690        &   good     & TI 800   \nl
1992  & Mar 7      & \nodata          & poor - blizzard  & TI 800  \nl
1992  & May 31     & \nodata           &  \nodata      & CCD out \nl
1992  & Aug 26-27  & A98 A160 A2462 c1919 & poor - clouds  & Loral 1 \nl
1992  & Dec 26 (half) & A98 A160 A690  &  ok     & Loral 2 \nl
1992  & Dec 27-28  &  \nodata          &  poor - clouds & Loral 2 \nl
1993  & Jan 21-24 (half) & A690 A1446 A1684 c1313 & great & Loral 2 \nl
1993  & Jul 22-23  & A160 c1919 A2214 a2462 & great & Loral 3 \nl
1993  & Sep 15-16 (half) & A98 A160 c1919 a2462 & good & Loral 3 \nl
\enddata
\label{mxlog}
\end{deluxetable}



==> tab3.tex <==
%auto-ignore
% Big data table for "Substructure in WAT Clusters:  New Redshifts and Analysis"
% 11/8/00 - stripped of stars/comments for astro-ph.

\newcommand{\kmsp}{~km~s$^{-1}$.\ }
\newcommand{\kmsc}{~km~s$^{-1}$,\ }
\newcommand{\kmse}{~km~s$^{-1}$!\ }

\begin{deluxetable}{crrrrrp{1in}}
\tablecaption{\sc Velocities and Positions of WAT Cluster Galaxies }
\tablehead{
\colhead{Gal. ID}     & \colhead{RA(2000)}   & \colhead{DEC(2000)} & 
\colhead{{\it cz}1\tablenotemark{a}}   & \colhead{{\it cz}2\tablenotemark{b}}  
& \colhead{$\epsilon$\tablenotemark{c}} & 
\colhead{NOTES\tablenotemark{d}}
}
\startdata
Abell 98 &          &         &        &    &     & \nl 
201  &  0 46 35.67  &  20 29 41.8  & 31999   &  \nodata  & 87 &  BGH337 \nl
202  &  0 46 29.33  &  20 28 04.4  & 30942   &  \nodata  & 42 & WAT, BGH401 \nl
203  &  0 46 36.26  &  20 28 26.3  & 32162   &  \nodata  & 44 & gE, BGH383 \nl
204  &  0 46 24.63  &  20 30 07.1  & 31261   &  \nodata  & 45 & BGH320? \nl
205  &  0 46 23.85  &  20 30 00.0  & 29895   &  \nodata  & 77 & BGH328? \nl
212  &  0 46 19.26  &  20 28 11.6  & 30453   &  \nodata  & 107 &  \nl
222  &  0 46 38.13  &  20 28 40.8  & 30981  &  \nodata  & 97 &  \nl
226  &  0 46 49.17  &  20 27 24.1  & 29315  &  \nodata  & 95 &  \nl
227  &  0 46 49.99  &  20 27 07.6  & 31643  &  \nodata  & 52 &  \nl
235  &  0 46 51.51  &  20 30 23.3  & 30547  &  \nodata  & 51 &  \nl
236  &  0 46 51.79  &  20 30 42.4  & 31852  &  \nodata  & 51 &  \nl
237  &  0 46 48.03  &  20 30 54.9  & 31066  &  \nodata  & 82 &  \nl
246  &  0 46 31.07  &  20 31 43.7  & 30991  &  \nodata  & 103 &  \nl
250  &  0 46 18.52  &  20 33 13.9  & 31519  &  \nodata  & 75 &  \nl
251  &  0 46 15.79  &  20 32 06.3  & 30691  &  \nodata  & 92 &  \nl
252  &  0 46 02.15  &  20 30 50.4  & 29872  &  \nodata  & 71 &  \nl
253  &  0 46 02.24  &  20 30 30.4  & 31770  &  \nodata  & 79 &  \nl
256  &  0 45 41.41  &  20 30 58.8  & 30890  &  \nodata  & 72 &  \nl
258  &  0 45 41.29  &  20 28 01.8  & 28811  &  \nodata  & 101 &  \nl
260  &  0 45 32.12  &  20 27 23.3  & 23715  &  \nodata  & 103 &  \nl
261  &  0 45 45.53  &  20 26 15.8  & 31267  &  \nodata  & 72 &  \nl
264  &  0 46 04.74  &  20 28 27.5  & 31612  &  \nodata  & 81 &  \nl
266  &  0 46 18.80  &  20 25 57.5  & 41346  &  \nodata  & 96 &  \nl
267  &  0 46 22.61  &  20 25 44.8  & 48228  &  \nodata  & 94 &  \nl
269  &  0 46 17.10  &  20 23 44.1  & \nodata  &  7277  & 200 &  \nl
270  &  0 46 14.69  &  20 23 41.9  & 31004  &  \nodata  & 48 &  \nl
271  &  0 46 28.46  &  20 23 47.9  & 30182  &  \nodata  & 66 &  \nl
272  &  0 46 33.92  &  20 23 54.6  & 32705  &  \nodata  & 45 &  \nl
275  &  0 46 37.02  &  20 26 06.1  & 30954  &  \nodata  & 90 &  \nl
279  &  0 46 38.55  &  20 22 53.3  & 31116  &  \nodata  & 59 &  \nl
281  &  0 46 35.19  &  20 20 31.0  & 30701  &  \nodata  & 51 &  \nl
282  &  0 46 28.17  &  20 21 05.3  & 36105  &  \nodata  & 96 &  \nl
283  &  0 46 33.24  &  20 14 57.1  & 35375  &  \nodata  & 88 &  \nl
286  &  0 46 48.95  &  20 15 29.4  & \nodata  &  15163  & 200 &  \nl
287  &  0 46 56.82  &  20 20 35.4  & 35554  &  \nodata  & 48 &  \nl
288  &  0 47 01.74  &  20 23 18.0  & em31439 &  \nodata   & 59 & stO2O3sHs Vab=31413 \nl
289  &  0 46 29.93  &  20 34 27.5  & \nodata  &  29315  & 200 &  \nl
291  &  0 46 52.58  &  20 25 23.3  & 32553  &  \nodata  & 100 &  \nl
295  &  0 47 09.39  &  20 29 17.0  & 31494  &  \nodata  & 82 &  \nl
297  &  0 47 23.22  &  20 31 21.5  & \nodata  &  4224  & 200 &  \nl
298  &  0 47 17.58  &  20 34 54.8  & 36861  &  \nodata  & 91 &  \nl
299  &  0 47 12.70  &  20 35 24.5  & 52979  &  \nodata  & 98 &  \nl
307  &  0 46 32.55  &  20 28 23.8  & 31766  &  \nodata  & 55 &  \nl
308  &  0 46 31.99  &  20 28 27.3  & 31431  &  \nodata  & 87 &  \nl
315  &  0 46 36.44  &  20 15 24.1  & 36160  &  \nodata  & 44 & BCG in A98Sb  \nl
316  &  0 46 47.61  &  20 11 23.4  & \nodata  &  36674  & 200 &  \nl
317  &  0 46 56.04  &  20 12 23.0  & 36970  &  \nodata  & 60 &  \nl
318  &  0 47 05.99  &  20 17 24.4  & 38919  &  \nodata  & 100 &  \nl
320  &  0 47 18.01  &  20 21 59.9  & 31451  &  \nodata  & 68 &  \nl
321  &  0 46 07.49  &  20 28 48.4  & 31734  &  \nodata  & 77 &  \nl
324  &  0 45 45.59  &  20 18 45.6  & 23221  &  \nodata  & 100 &  \nl
325  &  0 45 49.23  &  20 14 38.7  & 35977  &  \nodata  & 80 &  \nl
327  &  0 46 35.27  &  20 30 11.0  & 31203  &  \nodata  & 52 &  \nl
336  &  0 46 26.85  &  20 36 52.0  & 29831  &  \nodata  & 106 &  \nl
337  &  0 46 30.17  &  20 36 48.7  & 29380  &  \nodata  & 38 & BGH142,FD12 \nl
340  &  0 46 20.12  &  20 35 45.9  & 40217  &  \nodata  & 104 &  \nl
346  &  0 46 46.34  &  20 37 29.2  & \nodata  &  4644  & 200 &  \nl
348  &  0 46 44.64  &  20 37 00.5  & 37582  &  \nodata  & 98 &  \nl
351  &  0 46 45.56  &  20 40 12.6  & 40099  &  \nodata  & 75 &  \nl
352  &  0 46 44.47  &  20 40 23.9  & \nodata  &  36125  & 200 &  \nl
355  &  0 46 40.72  &  20 44 04.7  & 17288  &  \nodata  & 97 &  \nl
358  &  0 46 32.09  &  20 43 06.4  & 31358  &  \nodata  & 88 &  \nl
363  &  0 46 21.60  &  20 42 30.3  & 31354  &  \nodata  & 91 &  \nl
365  &  0 46 16.64  &  20 44 12.6  & \nodata  &  6611  & 200 &  \nl
368  &  0 46 07.52  &  20 40 59.4  & \nodata  &  45628  & 200 &  \nl
371  &  0 45 56.39  &  20 42 19.2  & \nodata  &  4814  & 200 &  \nl
376  &  0 45 57.44  &  20 36 55.2  & 30373  &  \nodata  & 75 &  \nl
378  &  0 46 07.86  &  20 38 47.0  & 31768  &  \nodata  & 58 &  \nl
388  &  0 46 56.51  &  20 27 04.8  & 30250  &  \nodata  & 66 &  \nl
392  &  0 46 15.51  &  20 33 19.1  & 30023  &  \nodata  & 48 &  \nl
393  &  0 46 18.45  &  20 32 28.6  & 58287  &  \nodata  & 104 &  \nl
394  &  0 46 23.41  &  20 32 14.5  & \nodata  &  41869  & 200 &  \nl
395  &  0 46 15.58  &  20 31 00.6  & 5787  &  \nodata  & 102 &  \nl
397  &  0 46 08.45  &  20 28 50.1  & 30371  &  \nodata  & 52 & O2,E+A BGH360 FD8 \nl
402  &  0 47 12.97  &  20 29 41.5  & 32044  &  \nodata  & 59 &  \nl
403  &  0 47 06.65  &  20 23 51.2  & 36484  &  \nodata  & 62 &  \nl
407  &  0 46 27.60  &  20 18 24.2  & 37169  &  \nodata  & 88 &  \nl
408  &  0 46 38.51  &  20 16 20.8  & 36630  &  \nodata  & 50 & \nl
413  &  0 47 25.80  &  20 10 02.8  & 37168  &  \nodata  & 90 &  \nl
414  &  0 46 34.36  &  20 11 57.4  & 35692  &  \nodata  & 58 &  \nl
415  &  0 46 27.67  &  20 10 41.5  & 36274  &  \nodata  & 70 &  \nl
416  &  0 46 20.25  &  20 08 13.4  & 35259  &  \nodata  & 66 &  \nl
419  &  0 46 29.24  &  20 14 04.6  & 36398  &  \nodata  & 92 &  \nl
420  &  0 46 16.29  &  20 16 12.5  & 37137  &  \nodata  & 83 &  \nl
421  &  0 45 59.01  &  20 15 29.2  & 38904  &  \nodata  & 78 &  \nl
423  &  0 45 57.47  &  20 12 56.0  & \nodata  &  61204  & 200 &  \nl
427  &  0 45 33.02  &  20 15 07.7  & 30062  &  \nodata  & 54 &  \nl
428  &  0 45 40.22  &  20 15 58.1  & 29947  &  \nodata  & 52 &  \nl
429  &  0 45 59.32  &  20 23 49.6  & 31713  &  \nodata  & 85 &  \nl
430  &  0 45 48.57  &  20 26 05.7  & 31146  &  \nodata  & 50 &  \nl
431  &  0 45 50.11  &  20 29 10.0  & 30324  &  \nodata  & 70 &  \nl
432  &  0 45 50.47  &  20 29 06.7  & 30966  &  \nodata  & 95 &  \nl
2080  &  0 46 20.70  &  20 29 06.0  & 30947  &  \nodata  & 44 &  \nl
0408  &  0 46 33.26  &  20 27 50.4  & 32456 &  \nodata  & 79 & BGH408 \nl
0396  &  0 46 31.89  &  20 28 09.5  & 32392 &  \nodata  & 69 & BGH396 \nl
0411  &  0 46 25.91  &  20 27 32.2  & 31199 &  \nodata & 100 & BGH411,FD10 \nl
0338  &  0 46 19.42  &  20 29 40.2  & 32855 &  \nodata  & 64 & BGH338 \nl
0311  &  0 46 16.00  &  20 30 18.5  & 31340 &  \nodata  & 53 & BGH311 \nl
0422  &  0 45 47.03  &  20 26 55.2  & 31260 &  \nodata  & 38 & BGH422 \nl
0353  &  0 46 21.93  &  20 29 04.8  & 33446 &  \nodata  & 40 & BGH353 \nl
0354  &  0 46 20.32  &  20 28 58.7  & 30387 &  \nodata  & 100 & BGH354,FD11 \nl
0125  &  0 46 24.78  &  20 37 17.3  & 30741 &  \nodata  & 39 & BGH125,radio \nl
0067  &  0 46 29.90  &  20 38 56.8  & 32609 &  \nodata  & 100 & BGH67,FD5 \nl
0092  &  0 46 15.94  &  20 38 07.7  & 32124 &  \nodata  & 49 & BGH92 \nl
0158  &  0 46 43.31  &  20 36 03.6  & 31336 &  \nodata  & 38 & BGH158,FD9 \nl
0221  &  0 46 29.66  &  20 33 17.0  & 31330 &  \nodata  & 100 & BGH221,FD6 \nl
0185  &  0 46 13.69  &  20 34 50.0  & 17523 &  \nodata  & 100 & BGH185,FD4 \nl
0184  &  0 46 04.06  &  20 34 50.0  & 30123 &  \nodata  & 45 & BGH184,FD13 \nl
0182  &  0 45 59.80  &  20 35 07.8  & 30772 &  \nodata  & 200 & BGH182 \nl
0175  &  0 45 52.86  &  20 35 11.4  & 10755 &  \nodata  & 37 & BGH175 \nl
0212  &  0 45 40.67  &  20 33 38.1  & 17965 &  \nodata  & 68 & BGH212 \nl
0030  &  0 46 08.12  &  20 40 43.3  & 30612 &  \nodata  & 51 & BGH30 \nl
0042  &  0 46 52.84  &  20 41 00.4  & 31497 &  \nodata  & 44 & BGH42 \nl
0095  &  0 47 14.01  &  20 38 09.8  & 18317 &  \nodata  & 80 & BGH95 \nl \hline
Abell 160 &          &        &     &   &    &  \nl 
201  &  1 12 59.64  &  15 29 27.4  & 13172  &  \nodata  & 100  & TJ \nl
202  &  1 12 59.94  &  15 29 29.4  & 12996  &  \nodata  & 80   &  \nl
203  &  1 13 03.73  &  15 30 07.1  & 12283  &  \nodata  & 62 &  \nl
204  &  1 12 58.68  &  15 28 13.9  & 12846  &  \nodata  & 59 &  \nl
205  &  1 12 57.66  &  15 28 19.7  & \nodata  &  3994  & 200 &  \nl
207  &  1 12 49.91  &  15 30 18.2  & 12800  &  \nodata  & 49 &  \nl
208  &  1 12 49.49  &  15 30 26.1  & 13596  &  \nodata  & 51 &  \nl
211  &  1 12 41.17  &  15 28 21.9  & 29460  &  \nodata  & 99 &  \nl
212  &  1 12 38.22  &  15 28 03.1  & 12807  &  \nodata  & 51 &  \nl
214  &  1 12 45.24  &  15 27 21.5  & 13234  &  \nodata  & 89 &  \nl
217  &  1 13 03.93  &  15 27 16.3  & 12388  &  \nodata  & 65 &  \nl
218  &  1 13 05.98  &  15 26 28.8  & 24400  &  \nodata  & 101 &  \nl
220  &  1 13 14.70  &  15 26 38.5  & em13912   &  \nodata  & 150 & O2O3sHs \nl
222  &  1 13 07.48  &  15 27 49.8  & 13080  &  \nodata  & 88 &  \nl
224  &  1 13 13.85  &  15 29 36.9  & \nodata  &  5197  & 200 &  \nl
225  &  1 13 16.28  &  15 30 09.5  & 13216  &  \nodata  & 54 &  \nl
226  &  1 13 15.64  &  15 30 25.0  & 14512  &  \nodata  & 46 &  \nl
227  &  1 13 13.26  &  15 30 27.3  & 12056  &  \nodata  & 65 &  \nl
228  &  1 13 15.73  &  15 30 58.2  & 14085  &  \nodata  & 20 &  \nl
229  &  1 13 07.47  &  15 30 30.8  & 13426  &  \nodata  & 75 &  \nl
230  &  1 13 02.89  &  15 31 37.5  & 13707  &  \nodata  & 41 &  \nl
231  &  1 13 00.16  &  15 31 50.3  &  2296  &  \nodata  & 103 &  \nl
233  &  1 12 54.08  &  15 32 47.8  & 13849  &  \nodata  & 45 &  \nl
234  &  1 12 48.04  &  15 31 42.2  & 12367  &  \nodata  & 44 &  \nl
236  &  1 12 38.04  &  15 33 02.4  & em12852 &  \nodata  & 77 & O2HsO3N2 Vab=12968 \nl
246  &  1 12 27.43  &  15 35 27.8  & 12578   &  \nodata   & 111 &  \nl
247  &  1 12 25.05  &  15 38 36.2  & 13367  &  \nodata  & 79 &  \nl
248  &  1 12 23.51  &  15 43 33.6  & 18281  &  \nodata  & 86 &  \nl
249  &  1 12 35.76  &  15 43 16.5  & em11376    &  \nodata  & 55   & O2HsO3 \nl
250  &  1 12 43.84  &  15 42 26.4  & 11618  &  \nodata  & 69 & O2O3HsN2 Vem=11615 \nl
251  &  1 12 40.87  &  15 39 29.9  & 2530  &  \nodata  & 104 &  \nl
253  &  1 13 16.50  &  15 40 35.5  & 11475  &  \nodata  & 86 & O2O3HsN2s Vem=11455 \nl
254  &  1 13 19.16  &  15 42 12.1  & 12980  &  \nodata  & 68 &  \nl
255  &  1 13 09.12  &  15 37 45.4  & 13441  &  \nodata  & 85 &  \nl
256  &  1 13 42.32  &  15 42 02.9  & \nodata  &   69522   & 200 &  \nl
257  &  1 13 45.01  &  15 40 59.2  & 13280  &  \nodata  & 60 & O2HsN2S2 Vem=13221 \nl
259  &  1 13 42.80  &  15 36 54.1  & 43762  &  \nodata  & 101 &  \nl
260  &  1 13 30.95  &  15 33 04.3  & 13303  &  \nodata  & 71 &  \nl
261  &  1 13 30.33  &  15 32 46.0  & 12024  &  \nodata  & 17 & H? \nl
262  &  1 13 34.51  &  15 32 24.0  & 18106  &  \nodata  & 60 &  \nl
264  &  1 13 40.92  &  15 31 52.5  & \nodata  &  23621  & 200 &  \nl
265  &  1 13 47.68  &  15 30 29.0  & 13561  &  \nodata  & 42 &  \nl
266  &  1 13 50.61  &  15 28 18.4  & 13054  &  \nodata  & 20 &  \nl
267  &  1 13 47.70  &  15 26 22.5  & 40233  &  \nodata  & 74 &  \nl
268  &  1 13 55.84  &  15 24 49.3  & 40134  &  \nodata  & 92 &  \nl
271  &  1 13 30.26  &  15 27 02.4  & \nodata  &  22908  & 200 &  \nl
272  &  1 13 16.40  &  15 23 35.1  & 13379  &  \nodata  & 107 &  \nl
273  &  1 13 21.52  &  15 21 02.8  & \nodata  &  40883  & 200 &  \nl
274  &  1 13 26.71  &  15 20 06.0  & 12570  &  \nodata  & 68 &  \nl
276  &  1 12 30.16  &  15 16 38.0  & \nodata  &  20387  & 200 &  \nl
278  &  1 12 13.97  &  15 16 36.8  & 13583  &  \nodata  & 214 &  \nl
282  &  1 12 24.47  &  15 20 07.2  & \nodata  &  12360    & 200 &  \nl
283  &  1 12 24.46  &  15 21 18.1  & 13146  &  \nodata  & 88 &  \nl
285  &  1 12 01.94  &  15 20 47.0  & \nodata  &  2576  & 200 &  \nl

292  &  1 12 44.03  &  15 35 20.5  & 13040  &  \nodata  & 87 &  \nl
293  &  1 12 53.96  &  15 36 07.6  & 12299  &  \nodata  & 47 &  \nl
294  &  1 12 59.52  &  15 35 28.6  & 12348  &  \nodata  & 42 & O2NeO3N2sHS2 Vem=12200 \nl
295  &  1 13 19.86  &  15 29 26.3  & em14649  &  \nodata  & 49   & O2O3HsN2 Vab=14858 \nl
296  &  1 12 13.60  &  15 42 47.4  & \nodata  &  33432  & 200 &  \nl
299  &  1 14 14.51  &  15 53 52.9  & 11365  &  \nodata  & 65 &  \nl
302  &  1 14 02.28  &  15 48 58.8  & 11466  &  \nodata  & 96 &  \nl
303  &  1 14 26.78  &  15 47 33.1  & em11856  &  \nodata  & 80 & O2O3sHsNe \nl
305  &  1 14 28.06  &  15 45 19.3  & 12559  &  \nodata  & 98 &  \nl
312  &  1 13 24.70  &  15 51 21.1  & \nodata  &  44888  & 200 &  \nl
313  &  1 13 21.96  &  15 51 04.2  & 13678  &  \nodata  & 50 &  \nl
314  &  1 13 11.92  &  15 49 59.2  & 13209  &  \nodata  & 47 &  \nl
315  &  1 13 29.98  &  15 48 56.6  & \nodata  &  29673  & 200 &  \nl
316  &  1 13 24.46  &  15 46 56.8  & 11480  &  \nodata  & 71 &  \nl
317  &  1 13 19.18  &  15 45 34.2  & 42490  &  \nodata  & 94 &  \nl
318  &  1 13 35.60  &  15 45 28.6  & 18079  &  \nodata  & 94 & Hs Vem=17919 \nl
320  &  1 13 45.36  &  15 47 31.4  & \nodata  &  22566  & 200 &  \nl
323  &  1 12 22.42  &  15 49 27.6  & 56704  &  \nodata  & 105 &  \nl
326  &  1 12 40.79  &  15 48 52.8  & 18110  &  \nodata  & 98 &  \nl
327  &  1 12 42.60  &  15 49 46.7  & \nodata  &  11127  & 200 &  \nl
328  &  1 12 27.41  &  15 44 59.0  & 11410  &  \nodata  & 42 &  \nl
329  &  1 12 20.13  &  15 46 02.4  & 18104  &  \nodata  & 89 &  \nl
330  &  1 12 22.35  &  15 44 19.0  & 18614  &  \nodata  & 66 &  \nl
331  &  1 12 29.93  &  15 44 18.8  & 11386  &  \nodata  & 103 &  \nl
332  &  1 12 01.65  &  15 45 22.8  & \nodata  &  20134  & 200 &  \nl
342  &  1 14 16.86  &  15 35 32.1  & 11472  &  \nodata  & 60 &  \nl
343  &  1 14 09.76  &  15 35 04.2  & 17910    &  \nodata  & 150 & HsN2 Vem=17814 \nl
361   &  1 15 12.57   &  15 24 37.3   &  36316   &   \nodata   & 100.8 &  \nl
363   &  1 15 21.13   &  15 18 29.2   &  36720   &   \nodata   &  95   &   \nl
364   &  1 15 30.75   &  15 17 15.5   &  36637   &   \nodata   &  40   &   \nl
366   &  1 15 08.95   &  15 17 31.0   &  20436   &   \nodata   &  62   &   \nl
368   &  1 14 58.98   &  15 20 57.9   &  20081   &   \nodata   &  61   &   \nl
369   &  1 15 01.19   &  15 21 20.9   &  20333   &   \nodata   &  69  & O2HsO3sO1N2 Vem=20310  \nl
370   &  1 14 35.19   &  15 20 53.6   &  \nodata &   20405     & 110   &   \nl
372   &  1 14 26.84   &  15 16 23.9   &  18428   &   \nodata   &  49   &   \nl
373   &  1 14 23.11   &  15 17 17.8   &  18332   &   \nodata   &  46   &   \nl
375  &  1 14 22.80  &  15 23 42.5  & 40508  &  \nodata  & 89 &  \nl
377  &  1 14 08.32  &  15 24 09.4  & em17976  &  \nodata  & 48   & O2O3HsN2S2 Vabs=18308 \nl
378  &  1 14 08.09  &  15 24 00.9  & \nodata  &  57542  & 200 &  \nl
382  &  1 14 33.50  &  15 30 09.4  & 13004  &  \nodata  & 100 &  \nl
383  &  1 14 35.30  &  15 30 49.6  & em18087 &  \nodata & 40 & O2HO3 \nl
384  &  1 14 51.45  &  15 29 35.0  & 19849  &  \nodata  & 74 &  \nl
385  &  1 14 36.45  &  15 26 25.6  & 31903  &  \nodata  & 102 &  \nl
387  &  1 14 53.96  &  15 41 27.4  & \nodata  &  15555  & 200 &  \nl
389  &  1 14 50.42  &  15 38 37.1  & \nodata  &  6970  & 200  &  \nl
395  &  1 14 10.18  &  15 43 28.1  & 23584  &  \nodata  & 99 &  \nl
396  &  1 14 07.45  &  15 43 33.7  & em18645  &  \nodata  & 51   & O2NeHO3s \nl
397  &  1 14 03.41  &  15 41 35.2  & 36418  &  \nodata  & 77 &  \nl
398  &  1 14 15.75  &  15 38 11.8  & 12808  &  \nodata  & 48 &  \nl
400  &  1 11 52.94  &  15 41 55.6  & 18244  &  \nodata  & 71 &  \nl
401  &  1 11 51.68  &  15 39 50.9  & 18069  &  \nodata  & 92 &  \nl
405  &  1 11 21.99  &  15 42 25.5  & 9661  &  \nodata  & 99 &  \nl
415  &  1 11 24.87  &  15 34 21.9  & 18667  &  \nodata  & 48 &  \nl
416  &  1 11 29.76  &  15 33 51.9  & 17871  &  \nodata  & 95 &  \nl
418  &  1 11 31.31  &  15 34 16.9  & \nodata  &  2146  & 200 &  \nl
420  &  1 11 48.58  &  15 34 12.0  & 1451  &  \nodata  & 97 &  \nl
421  &  1 11 56.60  &  15 27 58.2  & 13149  &  \nodata  & 56 &  \nl
422  &  1 11 53.33  &  15 28 10.8  & 12619  &  \nodata  & 90 &  \nl
425  &  1 11 50.22  &  15 21 01.4  & 17658  &  \nodata  & 71 &  \nl
427  &  1 11 28.21  &  15 22 05.4   &  25183   &   \nodata   &  100   &   \nl
432  &  1 15 39.52  &  15 14 42.6   & em16395  &   \nodata   &  40 & O2HsO3N2s \nl
435  &  1 15 13.45  &  15 12 45.2   &  20713   &   \nodata   &  64   &   \nl
438  &  1 14 22.43  &  15 14 48.5   &  18063   &   \nodata   &  44   &   \nl
442  &  1 14 21.33  &  15 07 21.9   &  18336   &   \nodata   &  32   &   \nl
444  &  1 14 32.34  &  15 08 28.8   &   \nodata   &  21305   &  200  &   \nl
445  &  1 14 17.33  &  15 03 35.7   &  18568   &   \nodata   &  98   &   \nl
448  &  1 14 36.05  &  14 59 29.4   &  18127   &   \nodata   &  76   &   \nl
453  &  1 15 08.42  &  14 54 02.3   &  21910   &   \nodata   &  89   &   \nl
462  &  1 15 20.89  &  15 02 27.9   &  38530   &   \nodata   &  91   &   \nl
465  &  1 14 45.96  &  15 06 07.6   &  13175   &   \nodata   &  107   &   \nl
468  &  1 13 26.20  &  15 15 05.4  & 12478  &  \nodata  & 95 &  \nl
469  &  1 13 24.35  &  15 14 27.2  & 12672  &  \nodata  & 95 &  \nl
471  &  1 12 36.45  &  15 11 47.6  & 59949  &  \nodata  & 103 &  \nl
473  &  1 12 28.63  &  15 11 01.3  & 42169  &  \nodata  & 96 &  \nl
480  &  1 12 50.06  &  15 02 03.5  & 17458  &  \nodata  & 81 &  \nl
482  &  1 12 21.90  &  15 00 37.9  & 8676  &  \nodata  & 87 &  \nl
484  &  1 12 20.48  &  14 58 00.7 &  11752  &   \nodata   &  94   &   \nl
491  &  1 13 11.99  &  15 05 58.0  & \nodata  &  45459  & 200 &  \nl
500  &  1 13 43.04  &  15 13 52.6  & 13609  &  \nodata  & 74 &  \nl
502   &  1 11 21.02   &  15 12 29.4   &   \nodata   &  51237   &  200  &   \nl
504   &  1 11 06.24   &  15 10 17.7   &  11457   &   \nodata   &  99   & HN2 Vem=11520  \nl
505   &  1 11 32.31   &  15 10 59.1   & em12042  &   \nodata   &  67   & O2O3sHsS2 \nl
508   &  1 11 48.01   &  15 05 53.1   & em11559  &   \nodata   &  40   & O2O3sHs \nl
511   &  1 11 36.63   &  15 04 41.0   &  41900   &   \nodata   &  76   &   \nl
512   &  1 11 26.78   &  15 07 50.2   &  18078   &   \nodata   &  104   &   \nl
514   &  1 11 25.92   &  15 01 02.0   &  18076   &   \nodata   &  44   &   \nl
515   &  1 11 50.95   &  15 03 44.2   & em39477   &   \nodata   &  52   & O2HsO3 \nl
516   &  1 11 46.27   &  14 58 39.2   &  13251   &   \nodata   &  58   &   \nl
517   &  1 11 54.68   &  14 56 51.3   &  42398   &   \nodata   &  91   &   \nl
519   &  1 11 09.81   &  14 54 10.7   & em18073  &   \nodata   &  78   & O2O3sHsN2 \nl
525   &  1 10 24.06   &  14 59 11.9   &  16409   &   \nodata   &  50   &   \nl
531   &  1 10 37.70   &  15 06 49.2   &   \nodata   &  18012   &  200  &   \nl
534   &  1 11 07.81   &  15 01 04.8   &  18303   &   \nodata   &  66  & O2HsN2s Vem=18394 \nl \hline
Abell 690  &         &        &     &   &    &  \nl 
1  &  8 39 15.83  &  28 50 38.5  & 23673  &  \nodata  & 75 & WAT \nl
2  &  8 39 14.67  &  28 50 10.7  & 24663  &  \nodata  & 81 &  \nl
3  &  8 39 10.75  &  28 49 21.4  & \nodata  &  14190  & 200 &  \nl
4  &  8 39 10.85  &  28 48 31.9  & 23253  &  \nodata  & 79 &  \nl
5  &  8 39 19.03  &  28 49 09.1  & 40353  &  \nodata  & 103 &  \nl
6  &  8 39 18.36  &  28 48 35.9  & 40115  &  \nodata  & 94 &  \nl
7  &  8 39 27.05  &  28 45 11.2  & 23552  &  \nodata  & 107 &  \nl
10  &  8 38 47.37  &  28 46 18.1  & 24333  &  \nodata  & 69 &  \nl
11  &  8 38 42.47  &  28 46 23.7  & 15370  &  \nodata  & 78 &  \nl
12  &  8 38 50.13  &  28 51 16.4  & 23646  &  \nodata  & 96 &  \nl
13  &  8 38 58.31  &  28 51 44.1  & 14448  &  \nodata  & 106 &  \nl
14  &  8 38 50.03  &  28 55 16.5  & 27623  &  \nodata  & 50 &  \nl
15  &  8 39 17.37  &  28 56 00.2  & 24685  &  \nodata  & 82 &  \nl
16  &  8 39 17.82  &  28 52 00.3  & 24536  &  \nodata  & 54 &  \nl
17  &  8 39 22.50  &  28 53 29.8  & 77610    &  \nodata  & 150  &  \nl
18  &  8 39 34.59  &  28 51 33.2  & \nodata  &  27556  & 200 &  \nl
19  &  8 39 32.96  &  28 51 02.3  & 23480  &  \nodata  & 398 &  \nl
20  &  8 39 41.30  &  28 53 52.8  & \nodata  &  22764  & 200 &  \nl
22  &  8 39 02.61  &  28 49 15.3  & 23346  &  \nodata  & 63 & O2O3s Vem=23349 \nl
24  &  8 39 37.17  &  28 48 34.9  & 23833  &  \nodata  & 147 &  \nl
25  &  8 39 38.66  &  28 47 19.5  & \nodata  &  25100  & 200 &  \nl
28  &  8 39 24.80  &  28 44 41.8  & 24207  &  \nodata  & 60 &  \nl
31  &  8 39 16.16  &  28 57 46.8  & 24296  &  \nodata  & 47 &  \nl
34  &  8 39 31.49  &  29 09 12.9  & 23534  &  \nodata  & 78 &  \nl
36  &  8 39 26.72  &  29 08 42.1  & 24097  &  \nodata  & 83 &  \nl
37  &  8 39 38.27  &  29 07 30.2  & 19829  &  \nodata  & 99 &  \nl
38  &  8 40 10.78  &  29 07 24.0  & 23938  &  \nodata  & 80 &  \nl
42  &  8 39 56.79  &  28 59 14.7  & 25202  &  \nodata  & 147 &  \nl
43  &  8 39 46.42  &  28 57 56.1  & 32386  &  \nodata  & 98 &  \nl
44  &  8 39 58.07  &  29 00 41.4  & 42538  &  \nodata  & 106 &  \nl
45  &  8 40 15.68  &  28 50 44.4  & 24280  &  \nodata  & 27 &  \nl
47  &  8 39 47.61  &  28 52 35.2  & 65794  &  \nodata  & 132 & O2? \nl
48  &  8 40 18.63  &  29 01 53.1  & 64343  &  \nodata  & 91 & O3s Vem=63684\nl
49  &  8 40 24.38  &  29 06 29.9  & 41654  &  \nodata  & 101 &  \nl
50  &  8 40 41.69  &  29 04 04.1  & 40696  &  \nodata  & 84 &  \nl
53  &  8 39 04.91  &  28 46 34.8  & 23402  &  \nodata  & 172 &  \nl
58  &  8 38 55.63  &  28 48 36.7  & \nodata  &  33944  & 200 &  \nl
61  &  8 39 32.45  &  28 41 27.4  & 24074  &  \nodata  & 148 &  \nl
62  &  8 39 37.75  &  28 41 54.0  & 24861  &  \nodata  & 102 &  \nl
63  &  8 39 40.16  &  28 42 28.3  & 24105  &  \nodata  & 75 &  \nl
64  &  8 39 51.05  &  28 41 19.9  & 40781  &  \nodata  & 79 &  \nl
65  &  8 39 47.48  &  28 43 37.0  & 23645  &  \nodata  & 89 &  \nl
67  &  8 40 09.56  &  28 50 15.6  & \nodata  &  40524  & 200 &  \nl
68  &  8 40 07.90  &  28 50 32.3  & 23828  &  \nodata  & 270 &  \nl
69  &  8 40 23.44  &  28 37 42.7  & 24513  &  \nodata  & 200 &  \nl
72  &  8 40 39.10  &  28 31 48.5  & 23892  &  \nodata  & 73 &  \nl
75  &  8 40 47.68  &  28 37 08.2  & \nodata  &  25092  & 200 &  \nl
76  &  8 40 31.92  &  28 41 06.7  & 50484    &  \nodata  & 144  & O2? \nl
77  &  8 40 55.03  &  28 43 48.2  & 24723  &  \nodata  & 65 &  \nl
82  &  8 39 09.28  &  28 49 24.0  & 24067  &  \nodata  & 32 &  \nl
83  &  8 39 08.96  &  28 59 46.0  & \nodata  &  31311  & 200 &  \nl
84  &  8 38 39.64  &  29 11 27.0  & 6245  &  \nodata  & 85 &  \nl
85  &  8 38 18.32  &  28 58 39.8  & 27957  &  \nodata  & 100 &  \nl
88  &  8 37 43.38  &  28 37 03.2  & 15483  &  \nodata  & 99 &  \nl
89  &  8 38 09.15  &  28 38 57.6  & 25194  &  \nodata  & 91 &  \nl
90  &  8 37 59.92  &  28 46 10.5  & \nodata  &  36932  & 200 &  \nl
91  &  8 38 22.35  &  28 48 28.8  & 40106  &  \nodata  & 203 &  \nl
92  &  8 38 19.69  &  28 47 23.8  & 2669  &  \nodata  & 103 &  \nl
93  &  8 38 35.77  &  28 44 22.0  & 23663  &  \nodata  & 49 &  \nl
95  &  8 38 22.68  &  28 41 35.4  & 15511  &  \nodata  & 111 &  \nl
97  &  8 38 23.09  &  28 38 55.9  & 15382  &  \nodata  & 58 &  \nl
98  &  8 38 39.84  &  28 38 31.3  & 23972  &  \nodata  & 54 &  \nl
99  &  8 38 27.40  &  28 32 26.1  & \nodata  &  14776  & 200 &  \nl
101  &  8 39 05.99  &  28 39 42.5  & 27782  &  \nodata  & 63 &  \nl
102  &  8 38 54.84  &  28 52 04.4  & 27651  &  \nodata  & 104 &  \nl
103  &  8 39 14.62  &  28 51 42.2  & 23074  &  \nodata  & 76 &  \nl
105  &  8 39 13.43  &  28 51 04.7  & 24052  &  \nodata  & 107 &  \nl
110  &  8 39 21.77  &  28 50 34.0  & 23992  &  \nodata  & 101 &  \nl
111  &  8 39 22.04  &  28 50 16.3  & 23734  &  \nodata  & 49 &  \nl
112  &  8 39 10.13  &  28 51 55.9  & 23635  &  \nodata  & 70 &  \nl
119  &  8 39 29.91  &  28 53 03.9  & 65593  &  \nodata  & 117 &  \nl
121  &  8 39 34.22  &  28 53 32.2  & 4648  &  \nodata  & 106 &  \nl
125  &  8 39 34.10  &  28 56 19.0  & 24347  &  \nodata  & 104 &  \nl
126  &  8 39 46.46  &  28 57 56.1  & 32043  &  \nodata  & 93 & O2HO3 Vem=32025 \nl
127  &  8 39 17.36  &  28 57 12.8  & 33469  &  \nodata  & 100 &  \nl
128  &  8 39 12.30  &  28 55 58.7  & \nodata  &  12234  & 200 &  \nl
129  &  8 39 05.74  &  28 57 12.1  & 41547  &  \nodata  & 102 &  \nl
130  &  8 38 48.18  &  28 56 01.4  & 28124  &  \nodata  & 35 &  \nl
131  &  8 39 02.03  &  28 55 32.0  & 24013  &  \nodata  & 91 &  \nl
135  &  8 39 47.25  &  28 50 47.5  & 38355  &  \nodata  & 95 &  \nl
136  &  8 39 09.90  &  28 42 45.9  & 23348  &  \nodata  & 94 &  \nl
140  &  8 38 52.33  &  28 37 59.1  & 24357  &  \nodata  & 53 &  \nl
141  &  8 38 24.56  &  28 39 40.4  & 16075  &  \nodata  & 72 &  \nl
142  &  8 38 11.37  &  28 39 39.8  & 25422  &  \nodata  & 65  & O2HO3 Vab=25117 \nl
143  &  8 38 23.78  &  28 41 07.1  & 23779  &  \nodata  & 78 &  \nl
145  &  8 38 37.84  &  28 44 13.9  & 24839  &  \nodata  & 98 &  \nl
146  &  8 38 34.27  &  28 48 15.3  & 40091  &  \nodata  & 76 &  \nl
147  &  8 38 36.82  &  28 48 00.2  & 23506  &  \nodata  & 116 &  \nl
149  &  8 38 40.73  &  28 49 37.7  & 24504  &  \nodata  & 117 &  \nl
151  &  8 38 12.65  &  28 57 40.9  & 23448  &  \nodata  & 68 &  \nl
152  &  8 38 15.08  &  28 58 07.3  & 7965  &  \nodata  & 107 &  \nl
154  &  8 38 24.97  &  28 59 46.3  & 28435  &  \nodata  & 101 &  \nl
155  &  8 38 32.86  &  29 00 38.5  & 24198  &  \nodata  & 88 &  \nl
158  &  8 38 53.84  &  28 57 53.7  & em24950 &  \nodata   & 32 & O2HO3 Vab=24574 \nl
161  &  8 39 06.72  &  29 00 26.8  & \nodata  &  54197  & 200 &  \nl
163  &  8 39 32.43  &  29 03 41.6  & 24456  &  \nodata  & 106 &  \nl
166  &  8 39 49.77  &  28 55 41.5  & \nodata  &  64573  & 200 &  \nl
168  &  8 39 56.22  &  28 50 10.7  & 65726  &  \nodata  & 51 &  \nl
170  &  8 40 16.50  &  28 49 13.9  & 23570  &  \nodata  & 56 &  \nl
171  &  8 40 07.99  &  28 47 43.3  & 63229  &  \nodata  & 83 &  \nl
174  &  8 39 50.89  &  28 48 16.3  & 40551  &  \nodata  & 129 &  \nl
177  &  8 40 08.16  &  28 43 55.9  & \nodata  &  15010  & 200 &  \nl
184  &  8 39 52.45  &  28 41 46.1  & 41073  &  \nodata  & 92 &  \nl
185  &  8 40 04.29  &  29 05 43.3  & 15278  &  \nodata  & 12 &  \nl
186  &  8 39 54.65  &  29 06 33.3  & em32195    &  \nodata  & 81   & O2HO3s Vab=32082 \nl
187  &  8 39 44.05  &  29 05 55.2  & 24327  &  \nodata  & 65 &  \nl
188  &  8 39 52.58  &  29 07 46.9  & 31357  &  \nodata  & 96 &  \nl
189  &  8 40 00.17  &  29 10 39.7  & 58218  &  \nodata  & 93 &  \nl
190  &  8 39 53.12  &  29 12 21.8  & 24234  &  \nodata  & 102 &  \nl
195  &  8 40 51.90  &  28 50 55.3  & 65840  &  \nodata  & 93 &  \nl
196  &  8 40 22.58  &  28 48 34.1  & \nodata  &  61936  & 200 &  \nl
408  &  8 39 42.40  &  28 34 57.3  & 23096  &  \nodata  & 62 &  \nl
409  &  8 39 32.90  &  28 28 40.5  & 29208  &  \nodata  & 73 &  \nl
411  &  8 39 13.41  &  28 35 57.9  & 28037  &  \nodata  & 102 &  \nl
414  &  8 38 43.91  &  29 07 02.4  & 40912  &  \nodata  & 75 &  \nl
415  &  8 38 47.43  &  29 11 10.9  & 44790  &  \nodata  & 101 &  \nl
420  &  8 37 40.62  &  28 50 00.0  & 31170  &  \nodata  & 95 &  \nl
421  &  8 37 42.61  &  28 47 54.2  & 24704  &  \nodata  & 99 &  \nl
422  &  8 37 42.84  &  28 46 11.2  & 17457  &  \nodata  & 83 &  \nl
423  &  8 38 05.26  &  28 42 37.9  & 30003  &  \nodata  & 49 &  \nl
424  &  8 38 45.76  &  28 35 40.4  & 24270  &  \nodata  & 90 &  \nl
425  &  8 39 13.41  &  28 35 57.9  & 27927  &  \nodata  & 106 &  \nl \hline
Abell 1446  &        &        &     &   &    &  \nl 
201  &  12 2 03.68  &  58 02 07.1  & 30826  &  \nodata  & 41 & WAT \nl
212  &  12 2 06.51  &  58 05 12.4  & 3542  &  \nodata  & 91 &  \nl
215  &  12 1 54.72  &  58 01 40.0  & 31026  &  \nodata  & 104 &  \nl
221  &  12 1 49.99  &  58 00 04.7  & 31233  &  \nodata  & 90 &  \nl
222  &  12 1 40.26  &  58 00 00.1  & 31641  &  \nodata  & 98 &  \nl
237  &  12 2 09.28  &  58 00 20.7  & 31577  &  \nodata  & 63 &  \nl
238  &  12 2 09.60  &  57 59 46.9  & em30317  &  \nodata  & 47 & O2HO3s \nl
243  &  12 2 15.66  &  58 00 40.8  & 29326  &  \nodata  & 95 &  \nl
246  &  12 2 21.95  &  58 04 41.9  & \nodata &  11247  & 200 &  \nl
251  &  12 1 55.70  &  57 58 15.3  & 30378  &  \nodata  & 53 &  \nl
252  &  12 1 16.03  &  57 59 00.2  & em32176  &  \nodata & 125 & O2HO3s \nl
254  &  12 1 46.58  &  57 57 02.3  & \nodata &  65236  & 200 &  \nl
255  &  12 1 41.60  &  57 57 05.6  & \nodata &  12087  & 200 &  \nl
259  &  12 2 00.40  &  57 55 39.7  & 17154  &  \nodata  & 93 &  \nl
260  &  12 2 13.29  &  57 57 10.9  & 30245  &  \nodata  & 42 &  \nl
266  &  12 2 30.87  &  57 55 11.1  & 30421  &  \nodata  & 80 &  \nl
268  &  12 2 13.52  &  57 53 31.1  & 61342  &  \nodata  & 93 &  \nl
270  &  12 1 40.12  &  57 52 46.6  & 37775  &  \nodata  & 85 &  \nl
271  &  12 1 38.44  &  57 52 32.4  & 31012  &  \nodata  & 89 &  \nl
275  &  12 0 28.86  &  57 52 10.9  & 45833  &  \nodata  & 88 &  \nl
276  &  12 0 37.97  &  57 53 37.2  & 30614  &  \nodata  & 90 &  \nl
283  &  12 0 15.74  &  57 59 38.7  & 30411  &  \nodata  & 50 &  \nl
289  &  12 1 06.14  &  58 00 10.6  & 30944  &  \nodata  & 28 &  \nl
291  &  12 1 30.74  &  58 02 01.0  & 30880  &  \nodata  & 72 &  \nl
292  &  12 1 28.46  &  58 02 48.8  & 19354  &  \nodata  & 64 &  \nl
293  &  12 1 24.73  &  58 03 23.3  & 4956   &  \nodata  & 99 &  \nl
294  &  12 1 30.77  &  58 03 26.4  & em30321 & \nodata  & 74 & O2NeHO3 \nl 
295  &  12 1 21.52  &  58 04 18.3  & 19642  &  \nodata  & 52 &  \nl
302  &  12 0 21.22  &  58 03 59.8  & \nodata  &  31808  & 200 &  \nl
305  &  12 0 35.60  &  58 07 48.5  & em10296  & \nodata   & 89 & O2HsO3N2 \nl
306  &  12 0 56.18  &  58 06 51.3  & 56182  &  \nodata  & 90 &  \nl
314  &  12 0 29.86  &  58 10 39.1  & 37983  &  \nodata  & 73 &  \nl
316  &  12 1 02.68  &  58 09 48.7  & 31110  &  \nodata  & 100 &  \nl
318  &  12 1 02.08  &  58 14 05.8  & 29603  &  \nodata  & 88 &  \nl
319  &  12 1 23.98  &  58 10 28.1  & 37782  &  \nodata  & 94 &  \nl
320  &  12 1 26.39  &  58 12 9.8  & 43565  &  \nodata  & 80 &  \nl
322  &  12 1 30.47  &  58 13 13.3  & 29513  &  \nodata  & 103 &  \nl
323  &  12 1 44.52  &  58 12 49.7  & em9774 &  \nodata  &  70 & O2O3HN2 \nl
326  &  12 1 38.28  &  58 07 25.4  & 44162  &  \nodata  & 99 &  \nl
329  &  12 1 46.97  &  58 07 11.2  & 12371  &  \nodata  & 34 &  \nl
330  &  12 1 49.78  &  58 05 53.5  & em12330 & \nodata  & 40 & stO2O3sH \nl
332  &  12 2 01.25  &  58 06 00.4  & 31573  &  \nodata  & 66 &  \nl
338  &  12 3 30.95  &  58 15 23.6  & em14834  & \nodata   & 46 & O2HsO3s \nl
340  &  12 3 26.60  &  58 11 33.7  & 37960  &  \nodata  & 100 &  \nl
345  &  12 2 58.85  &  58 12 56.0  & 37487  &  \nodata  & 61 &  \nl
353  &  12 1 55.90  &  58 11 10.7  & 30597  &  \nodata  & 100 &  \nl
354  &  12 2 21.67  &  58 07 05.8  & \nodata  &  30962  & 200 &  \nl
358  &  12 3 02.43  &  58 07 01.3  & 19774  &  \nodata  & 90 &  \nl
365  &  12 3 32.48  &  58 04 17.0  & 31736  &  \nodata  & 84 &  \nl
366  &  12 3 27.12  &  58 02 26.4  & 31260  &  \nodata  & 83 &  \nl
367  &  12 3 15.97  &  58 03 10.4  & 2288  &  \nodata  & 94 &  \nl
369  &  12 2 39.08  &  58 03 40.2  & 31476  &  \nodata  & 47 & O2O3 Vem=31655 \nl
372  &  12 2 39.54  &  58 01 18.7  & 30682  &  \nodata  & 56 &  \nl
373  &  12 2 41.22  &  58 00 43.7  & 30755  &  \nodata  & 45 &  \nl
374  &  12 3 06.12  &  58 00 43.3  & 31977  &  \nodata  & 93 &  \nl
376  &  12 3 45.62  &  57 59 22.3  & 31062  &  \nodata  & 107 &  \nl
380  &  12 3 20.68  &  57 55 15.8  & 31183  &  \nodata  & 135 &  \nl
383  &  12 3 13.37  &  57 53 53.2  & em10230 & \nodata  &  64 & stO2HO3sHsO1N2 Vab=10127 \nl
384  &  12 3 11.55  &  57 53 36.1  & \nodata  &  23941  & 200 &  \nl
385  &  12 3 13.83  &  57 53 23.4  & em10209  &  \nodata  & 70 & stO2NeHsO3sN2 Vab=10352 \nl
387  &  12 3 04.25  &  57 53 15.8  & \nodata  &  37104  & 200 &  \nl
390  &  12 2 55.72  &  57 51 58.7  & 30827  &  \nodata  & 56 &  \nl \hline
Abell 1684  &       &        &     &   &    &  \nl 
1  &  13 9 04.47  &  10 29 35.0  & 25961  &  \nodata  & 38 & WAT \nl
3  &  13 8 59.02  &  10 29 31.4  & 25993  &  \nodata  & 51 &  \nl
5  &  13 9 02.73  &  10 30 16.5  & 26445  &  \nodata  & 65 &  \nl
9  &  13 9 07.68  &  10 30 07.2  & \nodata  &  47346  & 200 &  \nl
10  &  13 9 07.79  &  10 29 54.8  & 25522  &  \nodata  & 44 &  \nl
11  &  13 9 11.47  &  10 27 50.7  & 25982  &  \nodata  & 68 &  \nl
13  &  13 8 53.05  &  10 28 26.5  & 26227  &  \nodata  & 90 &  \nl
15  &  13 8 56.83  &  10 30 42.8  & 26388  &  \nodata  & 75 &  \nl
17  &  13 8 54.79  &  10 31 14.3  & 25346  &  \nodata  & 30 & gE \nl
23  &  13 9 05.67  &  10 36 10.7  & 25222  &  \nodata  & 172 &  \nl
24  &  13 9 10.85  &  10 37 01.5  & 26160  &  \nodata  & 147 & gE \nl
25  &  13 9 22.07  &  10 35 18.7  & 26634  &  \nodata  & 89 &  \nl
26  &  13 9 31.67  &  10 36 00.3  & 26412  &  \nodata  & 71 &  \nl
29  &  13 9 18.83  &  10 31 52.6  & 30340  &  \nodata  & 76 &  \nl
31  &  13 9 32.80  &  10 28 11.3  & 25336  &  \nodata  & 74 &  \nl
32  &  13 9 21.32  &  10 26 57.7  & 47004  &  \nodata  & 61 &  \nl
34  &  13 9 18.86  &  10 24 29.6  & 25767  &  \nodata  & 43 &  \nl
35  &  13 9 13.81  &  10 23 29.5  & 16811  &  \nodata  & 85 & O2HO3s Vem=16859 \nl
39  &  13 8 44.75  &  10 27 32.0  & 26140  &  \nodata  & 81 &  \nl
41  &  13 8 43.09  &  10 30 05.5  & 25260  &  \nodata  & 135 &  \nl
43  &  13 8 29.07  &  10 30 57.3  & 33070  &  \nodata  & 106 &  \nl
45  &  13 8 08.99  &  10 34 40.3  & \nodata &  46932  & 200 &  \nl
46  &  13 8 31.28  &  10 33 19.2  & \nodata &  47324  & 200 &  \nl
47  &  13 8 31.02  &  10 35 35.7  & 26269  &  \nodata  & 86 &  \nl
50  &  13 8 28.61  &  10 40 08.1  & 7329  &  \nodata  & 35 & O2HsO3sN2 Vem=7339 \nl
52  &  13 9 09.86  &  10 37 17.9  & 26400  &  \nodata  & 94 &  \nl
54  &  13 9 17.69  &  10 40 24.7  & \nodata  &  9555  & 200 &  \nl
55  &  13 9 30.55  &  10 42 10.2  & 25551  &  \nodata  & 42 &  \nl
56  &  13 9 42.35  &  10 43 18.1  & 26781  &  \nodata  & 64 &  \nl
59  &  13 9 34.75  &  10 33 12.9  & 26432  &  \nodata  & 20 &  \nl
61  &  13 9 44.50  &  10 32 01.0  & 25663  &  \nodata  & 27 &  \nl
64  &  13 9 35.09  &  10 30 15.1  & 22625  &  \nodata  & 51 & O2HsO3s Vem=22596 \nl
65  &  13 9 55.26  &  10 29 39.2  & \nodata  &  25993  & 200 &  \nl
66  &  13 9 34.67  &  10 26 16.2  & 43373  &  \nodata  & 215 &  \nl
67  &  13 9 38.46  &  10 24 48.6  & 23966  &  \nodata  & 101 &  \nl
74  &  13 8 45.85  &  10 20 41.1  & 25985  &  \nodata  & 78 &  \nl
76  &  13 8 29.43  &  10 19 28.8  & 25557  &  \nodata  & 75 &  \nl
77  &  13 8 31.71  &  10 17 12.9  & em70490  &  \nodata  & 30 & O2HsO3s \nl
78  &  13 8 12.61  &  10 16 45.1  & 25812  &  \nodata  & 61 &  \nl
79  &  13 8 09.51  &  10 16 38.0  & 16598  &  \nodata  & 90 &  \nl
80  &  13 8 34.03  &  10 25 04.9  & 25660  &  \nodata  & 67 &  \nl
81  &  13 8 20.05  &  10 25 28.6  & 66440  &  \nodata  & 72 &  \nl
82  &  13 8 10.83  &  10 25 40.9  & 26037  &  \nodata  & 87 &  \nl \hline
1313+073 &          &        &     &   &    &  \nl 
1  &  13 16 17.02  &  7 02 46.6  & 15086  &  \nodata  & 76 & WAT \nl
2  &  13 16 21.16  &  6 59 38.5  & 14682  &  \nodata  & 68 &  \nl
3  &  13 16 03.35  &  7 04 50.7  & 6233  &  \nodata  & 98 &  \nl
5  &  13 16 12.92  &  7 01 28.5  & 25966  &  \nodata  & 81 &  \nl
6  &  13 16 15.24  &  7 03 03.4  & 15309  &  \nodata  & 96 &  \nl
7  &  13 16 12.68  &  7 01 48.4  & \nodata  &  13766  & 200 &  \nl
8  &  13 16 15.20  &  7 02 24.0  & 15043  &  \nodata  & 45 &  \nl
11  &  13 16 10.44  &  6 58 42.0  & \nodata  &  10722  & 200 &  \nl
12  &  13 16 07.78  &  6 58 32.3  & 14595  &  \nodata  & 124 &  \nl
13  &  13 16 01.25  &  7 01 15.8  & 16059  &  \nodata  & 124 &  \nl
14  &  13 16 19.69  &  6 56 22.2  & \nodata  &  24436  & 200 &  \nl
16  &  13 16 36.87  &  7 00 54.5  & 14269  &  \nodata  & 63 &  \nl
17  &  13 16 32.42  &  7 01 58.4  & 15607  &  \nodata  & 89 &  \nl
19  &  13 16 36.50  &  7 05 03.3  & 14777  &  \nodata  & 78 &  \nl
20  &  13 16 40.98  &  7 06 13.4  & 14159  &  \nodata  & 106 &  \nl
21  &  13 16 34.84  &  7 07 15.4  & 15232  &  \nodata  & 79 &  \nl
22  &  13 15 56.41  &  7 05 46.7  & 14336  &  \nodata  & 80 &  \nl
23  &  13 16 30.92  &  7 03 17.8  & 38630  &  \nodata  & 104 &  \nl
24  &  13 15 03.74  &  7 17 45.5  & 31586  &  \nodata  & 74 &  \nl
25  &  13 15 08.27  &  6 55 22.1  & 15695  &  \nodata  & 142 &  \nl
26  &  13 15 16.44  &  6 50 14.8  & 15536  &  \nodata  & 72 &  \nl
27  &  13 15 26.48  &  6 48 54.2  & \nodata  &  19885  & 200 &  \nl
29  &  13 15 33.38  &  6 42 19.1  & 27395  &  \nodata  & 88 &  \nl
32  &  13 15 00.39  &  6 52 15.6  & \nodata  &  3082  & 200 &  \nl
33  &  13 14 58.66  &  6 47 38.2  & 15719  &  \nodata  & 95 &  \nl
35  &  13 15 09.41  &  6 41 50.4  & 31524  &  \nodata  & 90 &  \nl
36  &  13 15 10.17  &  7 19 34.3  & \nodata  &  16497  & 200 &  \nl
37  &  13 15 19.90  &  7 19 05.5  & 13010  &  \nodata  & 139 &  \nl
42  &  13 14 53.52  &  7 14 19.6  & 13109  &  \nodata  & 69 &  \nl
43  &  13 16 16.97  &  7 02 57.5  & 14952  &  \nodata  & 40 &  \nl
45  &  13 16 10.07  &  7 02 36.9  & 14708  &  \nodata  & 62 &  \nl
48  &  13 16 17.03  &  6 37 52.3  & 14864  &  \nodata  & 90 &  \nl
49  &  13 17 03.83  &  6 42 41.9  & 1788  &  \nodata  & 101 &  \nl
50  &  13 17 22.17  &  6 50 31.7  & 15397  &  \nodata  & 56 &  \nl
51  &  13 17 46.75  &  6 36 55.8  & \nodata  &  8784  & 200 &  \nl
54  &  13 17 25.28  &  6 52 51.9  & 17757  &  \nodata  & 99 &  \nl
55  &  13 17 18.14  &  7 02 20.7  & 15689  &  \nodata  & 72 &  \nl
62  &  13 17 52.86  &  6 49 45.8  & 35584  &  \nodata  & 104 &  \nl
65  &  13 16 52.39  &  7 17 23.7  & 14768  &  \nodata  & 62 &  \nl
66  &  13 16 36.40  &  7 18 33.9  & 30808  &  \nodata  & 101 &  \nl
70  &  13 16 57.72  &  7 13 09.3  & 12790  &  \nodata  & 66 & O2HO3 Vem=12762 \nl
71  &  13 17 02.43  &  7 09 58.2  & 14321  &  \nodata  & 40 &  \nl
72  &  13 17 31.93  &  7 10 30.1  & \nodata  &  30141  & 200 &  \nl
73  &  13 17 36.00  &  7 18 01.5  & em13680  &  \nodata  & 54 & O2HO3s  \nl
74  &  13 18 06.38  &  7 07 38.0  & 14976  &  \nodata  & 57 & HO3s Vem=14907 \nl
76  &  13 16 27.62  &  7 02 06.0  & 15118  &  \nodata  & 73 &  \nl
80  &  13 16 16.02  &  7 06 50.0  & 15044  &  \nodata  & 52 &  \nl
83  &  13 16 36.97  &  7 05 09.4  & 14360  &  \nodata  & 43 &  \nl
86  &  13 16 03.34  &  6 56 29.9  & 15958  &  \nodata  & 74 &  \nl
87  &  13 16 11.51  &  7 00 12.3  & 15082  &  \nodata  & 57 &  \nl
92  &  13 15 46.54  &  6 59 48.2  & 57810  &  \nodata  & 98 &  \nl
95  &  13 15 08.64  &  6 58 37.0  & 15185  &  \nodata  & 100 &  \nl
100  &  13 15 24.69  &  6 54 43.7  & \nodata  &  20578  & 200 &  \nl
102  &  13 15 53.05  &  6 51 00.2  & 29065  &  \nodata  & 75 &  \nl
103  &  13 15 55.54  &  6 55 43.8  & \nodata  &  5894  & 200 &  \nl
104  &  13 15 53.68  &  6 42 14.3  & 15659  &  \nodata  & 99 &  \nl
106  &  13 16 17.03  &  6 37 52.3  & 15093  &  \nodata  & 39 &  \nl
107  &  13 15 26.74  &  6 35 32.4  & \nodata  &  24280  & 200 &  \nl
110  &  13 15 57.02  &  7 17 02.9  & em13206 & \nodata  &  64 & O2NeHO3s  \nl
112  &  13 14 56.46  &  7 04 11.5  & 13627  &  \nodata  & 82 &  \nl
113  &  13 16 08.27  &  7 26 30.7  & 13380  &  \nodata  & 66 &  \nl
114  &  13 15 26.20  &  7 25 02.1  & 31481  &  \nodata  & 79 &  \nl
116  &  13 15 03.11  &  7 29 06.1  & 27480  &  \nodata  & 102 &  \nl
121  &  13 14 28.34  &  7 29 34.3  & 28253  &  \nodata  & 96 &  \nl
122  &  13 16 00.49  &  6 47 19.3  & 15393  &  \nodata  & 63 &  \nl
130  &  13 15 53.58  &  6 41 05.0  & 15068  &  \nodata  & 77 &  \nl
131  &  13 16 05.47  &  6 35 47.1  & \nodata  &  41361  & 200 &  \nl
132  &  13 14 55.62  &  6 40 50.3  & 27785  &  \nodata  & 65 &  \nl
135  &  13 14 59.45  &  6 43 50.8  & 27400  &  \nodata  & 99 &  \nl
141  &  13 15 57.88  &  7 19 47.3  & 13512  &  \nodata  & 102 &  \nl
145  &  13 15 11.84  &  7 07 53.8  & 41465  &  \nodata  & 103 &  \nl
172  &  13 16 50.18  &  7 05 33.8  & em11958 & \nodata  & 67 & O2HsO3sN2 \nl
190  &  13 16 30.11  &  7 16 04.4  & \nodata  &  7500  & 200 &  \nl \hline
Abell 2214  &        &        &     &   &    &  \nl 
1  &  16 38 00.80  &  37 52 59.0  & 48526  &  \nodata  & 67 & WAT \nl
2  &  16 38 04.60  &  37 53 09.8  & 48626  &  \nodata  & 89 &  \nl
4  &  16 38 05.38  &  37 52 09.5  & 49210  &  \nodata  & 92 &  \nl
9  &  16 37 58.17  &  37 53 29.4  & 49453  &  \nodata  & 85 &  \nl
10  &  16 37 59.10  &  37 53 44.0  & 48278  &  \nodata  & 46 &  \nl
23  &  16 38 19.44  &  37 53 14.0  & 49634  &  \nodata  & 67 &  \nl
25  &  16 38 30.02  &  37 53 19.1  & 48884  &  \nodata  & 85 &  \nl
26  &  16 38 16.36  &  37 52 19.7  & 66273  &  \nodata  & 93 &  \nl
40  &  16 37 23.34  &  37 47 25.1  & 28788  &  \nodata  & 96 &  \nl
46  &  16 37 26.01  &  37 53 12.8  & 50208  &  \nodata  & 74 &  \nl
47  &  16 37 26.65  &  37 53 17.3  & 20871  &  \nodata  & 99 &  \nl
82  &  16 39 04.32  &  37 53 17.6  & 48514  &  \nodata  & 99 &  \nl
84  &  16 39 12.50  &  37 50 54.8  & 13983  &  \nodata  & 102 &  \nl
91  &  16 37 51.84  &  37 44 40.5  & 42029  &  \nodata  & 88 &  \nl
92  &  16 37 44.83  &  37 45 18.1  & 59317  &  \nodata  & 91 &  \nl
109  &  16 37 18.20  &  37 51 46.5  & 51109  &  \nodata  & 66 &  \nl
111  &  16 37 20.44  &  37 53 13.5  & 48623  &  \nodata  & 73 &  \nl
118  &  16 36 49.69  &  37 57 14.9  & 48510  &  \nodata  & 91 &  \nl
120  &  16 37 02.79  &  38 00 59.9  & 49631  &  \nodata  & 103 &  \nl
131  &  16 38 10.23  &  38 01 17.4  & 18725  &  \nodata  & 103 &  \nl
132  &  16 38 04.80  &  38 05 20.8  & 18552  &  \nodata  & 75 &  \nl
\hline
Abell 2220 &           &        &     &   &    &  \nl 
206  & 16 41 22.53  &  54 00 15.9  &  32081  & \nodata   &  81    & \nl
207  & 16 40 54.90  &  53 54 35.5  &  32791  & \nodata   &  86    & \nl
210  & 16 39 52.02  &  53 47 39.6  &  32083  & \nodata   &  56    & gE \nl
211  & 16 40 12.10  &  53 45 10.9  &  31479  & \nodata   &  60    & \nl
214  & 16 39 47.56  &  53 47 27.8  &  33392  & \nodata   &  83    & \nl
216  & 16 37 45.80  &  53 49 23.4  &  31691  & \nodata   &  78    & \nl
217  & 16 37 11.04  &  53 47 49.8  & \nodata  &  22055   & 200    & \nl
218  & 16 37 42.11  &  53 47 29.5  &  30506  & \nodata   &  65    & \nl
220  & 16 38 33.30  &  53 46 22.2  &  30682  & \nodata   &  94    & \nl
224  & 16 37 45.94  &  53 50 43.5  &  32026  & \nodata   &  105    & \nl
225  & 16 38 52.69  &  53 55 56.4  &  30406  & \nodata   &  74    & \nl
226  & 16 39 32.63  &  53 46 43.6  &  32991  & \nodata   &  63    & WAT \nl
228  & 16 39 19.57  &  53 47 43.5  &  32261  & \nodata   &  66    & \nl
229  & 16 39 25.76  &  53 45 45.1  &  37045  & \nodata   &  89    & \nl
230  & 16 39 34.80  &  53 48 42.9  &  33466  & \nodata   &  63    & \nl
233  & 16 38 50.21  &  53 53 13.1  & \nodata  &  43979   &  200   & \nl
234  & 16 38 14.68  &  54 01 48.0  &  38751  & \nodata   &  97    & \nl
239  & 16 39 13.61  &  54 00 45.2  &  31354  & \nodata   &  96    & \nl
246  & 16 39 20.28  &  54 06 35.3  &  28453  & \nodata   &  88    & \nl
247  & 16 38 03.65  &  54 04 49.9  &  20638  & \nodata   &  43    & \nl
250  & 16 40 55.59  &  53 31 26.0  & \nodata  &  14685   &  200   & \nl
272  & 16 38 46.49  &  53 35 34.4  &  32723  & \nodata   &  46    & \nl
287  & 16 38 36.95  &  53 43 38.1  &  32430  & \nodata   &  82    & \nl
292  & 16 39 37.37  &  53 45 36.3  &  32574  & \nodata   &  105    & \nl
293  & 16 39 54.43  &  53 44 55.9  &  36964  & \nodata   &  80    & \nl
294  & 16 39 52.95  &  53 44 00.4  &  31717  & \nodata   &  87    & \nl
\hline
Abell 2462 & (= A3897) &        &          &   &    &  \nl 
1  &  22 39 11.42  &  -17 20 28.7  & 22233  &  \nodata  & 39 & WAT, enacs8  \nl
2  &  22 39 10.72  &  -17 20 26.1  & 22078  &  \nodata  & 96 &  \nl
4  &  22 39 10.42  &  -17 20 06.9  & 64660  &  \nodata  & 104 &  \nl
5  &  22 39 08.72  &  -17 20 00.5  & 23631  &  \nodata  & 83 &  \nl
7  &  22 39 12.57  &  -17 19 21.6  & 22210  &  \nodata  & 56 &  \nl
13  &  22 39 10.55  &  -17 21 30.7  & 22971  &  \nodata  & 86 &  \nl
14  &  22 39 09.73  &  -17 22 15.3  & 21610  &  \nodata  & 47 & enacs7 \nl
20  &  22 39 17.98  &  -17 20 13.0  & 21944  &  \nodata  & 54 &  \nl
24  &  22 39 19.41  &  -17 17 38.5  & \nodata  &  21051  & 200 &  \nl
27  &  22 39 12.25  &  -17 17 14.6  & 22543  &  \nodata  & 41 &  \nl
28  &  22 39 11.45  &  -17 17 31.5  & 21465  &  \nodata  & 64 &  \nl
29  &  22 39 12.81  &  -17 17 42.9  & 21304  &  \nodata  & 35 &  \nl
36  &  22 39 00.64  &  -17 20 29.3  & 35868  &  \nodata  & 75 &  \nl
38  &  22 38 51.97  &  -17 21 14.4  & 22428  &  \nodata  & 52 &  \nl
41  &  22 39 01.90  &  -17 22 54.9  & \nodata  &  4159  & 200 &  \nl
43  &  22 39 05.88  &  -17 23 04.0  & 21471  &  \nodata  & 45 & enacs5 \nl
48  &  22 38 52.01  &  -17 23 51.8  & 35969  &  \nodata  & 90 &  \nl
50  &  22 38 48.13  &  -17 26 25.2  & 14715  &  \nodata  & 66 & enacs3 \nl
51  &  22 38 29.33  &  -17 27 08.9  & 21448  &  \nodata  & 84 & enacs1, O3sHN2 Vem=21384 \nl
53  &  22 38 40.65  &  -17 29 44.7  & \nodata  &  10200  & 200 &  \nl
57  &  22 38 53.38  &  -17 29 02.6  & 37652  &  \nodata  & 88 &  \nl
58  &  22 39 01.06  &  -17 26 49.0  & 22044  &  \nodata  & 89 &  \nl
59  &  22 39 09.53  &  -17 25 43.7  & 21492  &  \nodata  & 40 &  \nl
61  &  22 39 06.86  &  -17 28 19.8  & 21592  &  \nodata  & 98 &  \nl
62  &  22 39 06.70  &  -17 29 09.9  & 29873  &  \nodata  & 79 &  \nl
63  &  22 39 04.61  &  -17 31 12.8  & 53126  &  \nodata  & 96 &  \nl
64  &  22 39 16.78  &  -17 30 15.3  & 22419  &  \nodata  & 48 &  \nl
66  &  22 39 25.70  &  -17 30 33.2  & 29997  &  \nodata  & 87 & enacs11 \nl
72  &  22 39 46.57  &  -17 30 41.6  & \nodata  & em21792 & 200 & wkO2HO3 \nl
77  &  22 39 33.21  &  -17 24 18.7  & 62337  &  \nodata  & 74 &  \nl
78  &  22 39 45.55  &  -17 24 42.1  & 22227  &  \nodata  & 97 &  \nl
80  &  22 39 55.51  &  -17 24 19.6  & 14934  &  \nodata  & 80 & enacs12 \nl
83  &  22 39 23.75  &  -17 23 47.6  & 23607  &  \nodata  & 67 &  \nl
88  &  22 39 33.54  &  -17 20 11.6  & 21966  &  \nodata  & 75 &  \nl
89  &  22 39 33.86  &  -17 21 18.4  & 53960  &  \nodata  & 96 &  \nl
91  &  22 39 42.17  &  -17 20 50.6  & 23360  &  \nodata  & 66 &  \nl
93  &  22 39 48.15  &  -17 21 49.5  & 23108  &  \nodata  & 76 &  \nl
101  &  22 39 34.43  &  -17 18 20.9  & 22156  &  \nodata  & 44 &  \nl
102  &  22 39 39.52  &  -17 17 53.8  & \nodata  &  17025  & 200 &  \nl
112  &  22 39 52.27  &  -17 11 29.8  & 54267  &  \nodata  & 68 &  \nl
114  &  22 39 38.10  &  -17 13 16.6  & 15802  &  \nodata  & 102 &  \nl
115  &  22 39 25.63  &  -17 09 50.8  & 22676  &  \nodata  & 91 &  \nl
117  &  22 39 22.73  &  -17 11 58.0  & \nodata  &  1375  & 200 &  \nl
118  &  22 39 21.34  &  -17 12 33.1  & 21469  &  \nodata  & 46 & enacs10 \nl
119  &  22 39 23.61  &  -17 15 39.3  & \nodata  &  63998  & 200 &  \nl
120  &  22 39 20.93  &  -17 16 15.5  & 21442  &  \nodata  & 102 &  \nl
126  &  22 39 06.26  &  -17 15 40.7  & 22345  &  \nodata  & 62 &  \nl
130  &  22 39 02.69  &  -17 11 35.7  & 38023  &  \nodata  & 77 &  \nl
135  &  22 38 53.55  &  -17 11 15.6  & 22719  &  \nodata  & 47 & enacs4 \nl
144  &  22 38 46.32  &  -17 16 36.1  & 22677  &  \nodata  & 80 & O2? \nl
152  &  22 38 35.99  &  -17 19 58.6  & 21955  &  \nodata  & 62 & enacs2 \nl
156  &  22 38 30.43  &  -17 21 41.0  & \nodata  &  8648  & 200 &  \nl
157  &  22 38 37.37  &  -17 21 30.8  & \nodata  &  38083  & 200 &  \nl
158  &  22 38 36.49  &  -17 22 40.7  & \nodata  &  23178  & 200 &  \nl
163  &  22 38 04.21  &  -17 17 20.5  & \nodata  &  8386  & 200 &  \nl
164  &  22 38 21.25  &  -17 21 34.6  & \nodata  &  7635  & 200 &  \nl
167  &  22 38 16.90  &  -17 23 13.7  & 23763  &  \nodata  & 99 &  \nl
169  &  22 38 00.70  &  -17 25 10.4  & \nodata  &  34728  & 200 &  \nl
173  &  22 37 38.48  &  -17 27 44.3  & 6683  &  \nodata  & 89 &  \nl
174  &  22 37 37.92  &  -17 28 09.8  & 27706  &  \nodata  & 72 &  \nl
178  &  22 37 22.43  &  -17 23 53.6  & 21012  &  \nodata  & 84 &  \nl
180  &  22 37 27.31  &  -17 22 11.8  & 20700  &  \nodata  & 56 &  \nl
192  &  22 37 23.32  &  -17 18 06.3  & \nodata  &  24089  & 200 &  \nl
194  &  22 38 39.10  &  -17 32 29.3  & em20808 &  \nodata & 74 & O2NeHs \nl
196  &  22 38 59.14  &  -17 33 55.6  & 17001  &  \nodata  & 101 &  \nl
197  &  22 39 17.78  &  -17 32 28.8  & \nodata &  22133 & 200 &  \nl
401  &  22 39 56.42  &  -17 34 12.6  & 8077  &  \nodata  & 106 &  \nl
404  &  22 39 32.55  &  -17 34 58.0  & 31353  &  \nodata  & 81 &  \nl
409  &  22 39 20.29  &  -17 37 20.2  & 22361  &  \nodata  & 62 & enacs9 \nl
410  &  22 39 06.69  &  -17 36 51.2  & 23161  & \nodata  & 81 & enacs6 \nl
414  &  22 38 25.52  &  -17 38 29.1  & em22012 & \nodata & 63 & O2O3O1H \nl
416  &  22 38 55.69  &  -17 41 36.4  & \nodata &  30760  & 200 &  \nl
439  &  22 38 32.87  &  -17 43 04.1  & 43023  &  \nodata  & 97 &  \nl
462  &  22 40 08.65  &  -17 15 56.7  & 28388  &  \nodata  & 72 &  \nl
463  &  22 40 10.91  &  -17 19 22.0  & 22424  &  \nodata  & 84 &  \nl
467  &  22 40 06.46  &  -17 22 38.6  & 22879  &  \nodata  & 68 &  \nl
468  &  22 40 22.67  &  -17 24 01.9  & 22952  &  \nodata  & 74 &  \nl
471  &  22 40 08.74  &  -17 24 36.2  & 22497  &  \nodata  & 83 & enacs13 \nl
473  &  22 40 30.99  &  -17 25 08.5  & 53217  &  \nodata  & 68 &  \nl
475  &  22 40 28.28  &  -17 27 36.9  & 22590  &  \nodata  & 90 &  \nl
488  &  22 39 36.56  &  -17 07 42.2  & 22343  &  \nodata  & 56 &  \nl
489  &  22 39 32.44  &  -17 07 54.2  & 21858  &  \nodata  & 42 &  \nl
490  &  22 39 30.33  &  -17 07 11.5  & \nodata & em23385  & 200 & wkO1N2HS2 \nl
496  &  22 39 55.85  &  -16 58 26.2  & 19053  &  \nodata  & 107 &  \nl
500  &  22 39 14.78  &  -17 00 25.7  & \nodata  &  23151  & 200 &  \nl
504  &  22 38 57.15  &  -17 02 47.9  & 31769  &  \nodata  & 96 &  \nl
506  &  22 39 15.90  &  -17 05 52.8  & \nodata  &  21481  & 200 &  \nl
510  &  22 39 00.07  &  -17 06 59.5  & 34177  &  \nodata  & 107 &  \nl
516  &  22 38 48.60  &  -17 08 40.2  & 22060  &  \nodata  & 81 &  \nl
517  &  22 38 35.25  &  -17 06 24.8  & \nodata  &  10193  & 200 &  \nl
565  &  22 38 11.91  &  -17 04 54.9  & 22550  &  \nodata  & 75 &  \nl
571  &  22 37 41.49  &  -17 06 01.1  & 27969  &  \nodata  & 104 &  \nl
586  &  22 40 21.07  &  -17 38 12.5  & 22460  &  \nodata  & 53 &  \nl
608  &  22 37 58.50  &  -17 35 49.7  & 41243  &  \nodata  & 94 &  \nl
\enddata
\tablenotetext{a}{Category 1 heliocentric velocity in \kmsp  Velocities 
beginning in "em'' are measured from emission lines.  }
\tablenotetext{b}{Category 2 heliocentric velocity in \kmsp }
\tablenotetext{c}{Velocity error in \kmsc see text. }
\tablenotetext{d}{Key to NOTES: WAT - wide-angle tailed radio galaxy;
TJ - Twin Jet morphology; FD - id from Faber \& Dressler 1977; BGH -
id from Beers, Geller, \& Huchra 1982; gE - giant elliptical, usually
2nd ranked in cluster.  }
\tablenotetext{~}{
The following codes pertain to the emission line survey: 
H  = hydrogen Balmer line; O3 = [OIII] 4363, 4959 or 5007\AA ; 
O2 = [OII] 3727\AA; O1 = [OI] 6300\AA; N1 = [NI] 5199\AA; 
N2 = [NII] 6548 or 6583\AA ; Ne = [NeIII] 3869\AA ;
E+A = strong H absorption blueward of Ca lines ;
s = pluralizes the preceding code to refer to 2 or more lines from
a species; em = emission; ab = absorption; st = strong; wk = weak; 
? = uncertain.
Absorption line velocities are placed in the notes column if they
are significantly less certain than the emission line velocity. }
\label{bigtab}
\end{deluxetable} 


==> tab4.tex <==
%auto-ignore
% 6/4/96 Follow the sample tables in AASTEX.  For use with the
% style "aj_pt4.sty", and the master file "tables.tex".
% 6/15/00 - cp watdyn.tex means.tex
%	    This will just give the mean and stddev for each new
%           WAT database in Paper I.

\newcommand{\kms}{\ifmmode \hbox{ \rm km s}^{-1} \else{ km s$^{-1} $}\fi}

\begin{deluxetable}{lrrcc}
\tablecaption{\sc Traditional Velocity Data for WAT Clusters } 
\tablehead{
\colhead{Cluster}   &  \colhead{N$_{tot}$}  &   \colhead{N$_{Memb}$}        
& \colhead{V$_{\mu}$} &  \colhead{S$_\sigma$}    \\
 \colhead{Name} &   &   & \colhead{\kms} & \colhead{\kms}  
}
\startdata
A98(N+S)  & 101 & 69  & 31,085$\pm 96$ & 797$\pm73$    \nl
A160      & 125 & 65  & 12,814$\pm102$ & 1062$\pm144$   \nl
A690      & 106 & 57  & 24,109$\pm 69$ & 950$\pm217$   \nl
A1446     &  54 & 31  & 30,865$\pm112$ & 616$\pm83$   \nl
A1684     &  38 & 29  & 25,791$\pm 79$ & 760$\pm246$   \nl
Cl1313+073 & 60 & 43  & 14,742$\pm128$ & 999$\pm142$   \nl
A2214     &  21 & 13  & 49,139$\pm156$ & 706$\pm197$   \nl
A2220     &  23 & 19  & 32,274$\pm199$ & 1297$\pm488$   \nl
A2462     &  74 & 48  & 22,172$\pm 97$ & 784$\pm133$   
\tablecomments{$V_{\mu}$ is the mean of the velocities within 4000 \kms of
the WAT velocity.  There is no clipping or correction for substructure in 
these velocity samples.  $S_{\sigma}$ is the velocity dispersion as estimated by
the standard deviation  with a cosmological correction factor of (1+z)$^{-1}$.
}
\label{means}
\enddata
\end{deluxetable}



==> tab5.tex <==
%auto-ignore
% \documentstyle[12pt]{article}
% vcomp.tex - comparison of velocity measurements of WAT clusters.
% This will be compatible
% with "aj_pt4.sty" (AASTEX).

\def\kms{\ifmmode \hbox{ \rm km s}^{-1} \else{ km s$^{-1} $}\fi}

\begin{deluxetable}{lrlrc}
\tablecaption{\sc Comparison of Galaxy Velocities }
\tablehead{
\colhead{Galaxy ID} & \colhead{cz$_{us}$}   & \colhead{cz$_{ref}$} & 
\colhead{$\Delta$ cz}      & \colhead{References}  \\
\colhead{ } & \colhead{\kms}  & \colhead{\kms}  &\colhead{\kms} &
\colhead{ }
}
\startdata
A98 203 & 32162$\pm$44 & 32041$\pm$48 &  121 & 1 \nl
        &              & 32070$\pm$51 &   92 & 2 \nl
A98 202 & 30942$\pm$42 & 30989$\pm$40 &  -47 & 1 \nl
        &              & 31001$\pm$46 &  -59 & 2 \nl
A98 201 & 32000$\pm$88 & 32164$\pm$202 & -164 & 1 \nl
        &              & 31710$\pm$91 &  290 & 2 \nl
A98 204 & 31262$\pm$45 & 31351$\pm$54 &  -89 & 1 \nl
        &              & 31367$\pm$55 & -105 & 2 \nl
A98 205 & 29895$\pm$78 & 29860$\pm$53 &   35 & 1 \nl
        &              & 29910$\pm$54 &  -15 & 2 \nl
A98 397 & 30371$\pm$53 & 30565$\pm$100 & -193 & 3 \nl
A98 337 & 29380$\pm$38 & 29512$\pm$100 & -132 & 3 \nl
A2462 50 & 14715$\pm$67  & 14746$\pm$54 & 31  &  4 \nl
A2462 66 & 29998$\pm$88  & 29817$\pm$81 & -181 & 4  \nl
A2462 51 & 21449$\pm$85  & 21414$\pm$78 & -35  & 4  \nl
A2462 152 & 21955$\pm$62 & 21988$\pm$57 & 33   & 4  \nl
A2462 135 & 22720$\pm$48 & 22369$\pm$87 & -351 & 4  \nl
A2462 43 & 21471$\pm$45  & 21311$\pm$75 & -160 & 4  \nl
A2462 410 & 23162$\pm$82 & 23147$\pm$60 & -15  & 4  \nl
A2462 14 & 21610$\pm$48  & 21578$\pm$63 & -32  & 4  \nl
A2462 1  & 22234$\pm$39  & 22198$\pm$57 & -36  & 4  \nl
A2462 409 & 22361$\pm$62 & 22208$\pm$60 & -153 & 4  \nl
A2462 118 & 21469$\pm$47 & 21350$\pm$63 & -119 & 4  \nl
A2462 471 & 22498$\pm$83 & 22330$\pm$63 & -168 & 4  
\tablenotetext{ }{}
\tablerefs{ (1) Beers, Geller \& Huchra 1982 (BGH),
(2) Zabludoff, Huchra, \& Geller 1990, (3) Faber \& Dressler 1977,
(4) Katgert, Mazure, den Hartog, Adami, Biviano, \& Perea (1998).
}
\enddata
\end{deluxetable}




==> tab6.tex <==
% elgs.tex - table of results of emission line galaxy survey
% 4/27/00 - copy of mxlog.tex
% Use style "aj_pt4.sty", and the master file "tables.tex".

\begin{deluxetable}{llcccll}
\tablecaption{\sc Emission Line Galaxy Counts} 
\tablehead{
\colhead{Cluster}   & \colhead{z\tablenotemark{1}} & 
\colhead{Members\tablenotemark{2}}  & 
\colhead{\%ELGs\tablenotemark{3}}  & \colhead{\%ELGs Non-mem\tablenotemark{4}} &
\colhead{H$\alpha$\tablenotemark{5}} &  \colhead{Comments\tablenotemark{6}}
}
\startdata
Abell   98 & 0.1037 &  53\tablenotemark{a} &  1.9(1/53)  &  0.0(0/28) & 7261\AA & NS interferes w/OIII\nl
Abell  160 & 0.0427 &  65  &  20.0(13/65)  & 15.0(9/60)  & 6852\AA & NS interferes w/H$\beta$ \nl
Abell  690 & 0.0804 &  56  &  5.4(3/56)  &  6.0(3/50) & 7088\AA & \nl
Abell 1446 & 0.1029 &  30  &  13.3(4/30)  & 24.0(6/25) & 7240\AA & NS interferes w/OIII \nl
Abell 1684 & 0.0860 &  29  &  3.4(1/29)  & 33.3(3/9) & 7131\AA & NS interferes w/H$\beta$ and MgB \nl
Cl1313+073 & 0.0492 &  42  &  9.5(4/42)  &  0.0(0/17) & 6890\AA & NS interferes w/H$\beta$  \nl
Abell 2214 & 0.1639 &  13  &  0.0(0/13)  &  0.0(0/8)  & 7634\AA & \nl
Abell 2462 & 0.0739 &  48  &  6.3(3/48)  &  0.0(0/24)  & 7050\AA & NS interferes w/H$\beta$ and MgB \nl
\tableline
TOTAL      & \nodata & 336 & 8.6(29/336) &  9.5(21/221)  & \nodata & \nodata 
\tablenotetext{1}{Derived from V$_{\mu}$ in Table 4.}
\tablenotetext{2}{Members include only C1 velocities within $\approx$ 4000 \kms of 
the WAT's velocity.} 
\tablenotetext{3}{Percentage of member, C1 galaxies with emission lines.}
\tablenotetext{4}{Percentage of non-member, C1 galaxies with emission lines.}
\tablenotetext{5}{Redshifted wavelength of H$\alpha$. } 
\tablenotetext{6}{NS = night sky emission line. The 5577\AA\ and 5195\AA\
NS lines were especially problematic.  } 
\tablenotetext{a}{Does not include members adopted from literature.} 
\enddata
\label{elg}
\end{deluxetable}


==> tab7.tex <==
%auto-ignore
% spatial.tex - table of results of emission line galaxy survey
% 5/1/00 - copy of elgs.tex
% Use style "aj_pt4.sty", and the master file "tables.tex".

% Sampling counts and factors that influence the counts.
% Cluster R searchfield NoExposures   Multicol{subregions} TotCand. ObsCand. TotPerc Fair?
%                                    Quad1 Quad2 Quad3 Quad4 In Outer
%                   12345678901234
\begin{deluxetable}{lccrccccccccll}
\tablecaption{\sc Spatial Uniformity of MX Observations} 
\tablehead{
\colhead{Cluster}   & \colhead{R\tablenotemark{1}} & 
\colhead{Field\tablenotemark{2}} & \colhead{N$_{exp}$\tablenotemark{3}} & 
\colhead{Q1\tablenotemark{4}} & \colhead{Q2} & \colhead{Q3} & \colhead{Q4} & 
\colhead{In} & \colhead{Out}  &
\colhead{N$_{Cand.}$\tablenotemark{5}} &  \colhead{N$_{Samp}$\tablenotemark{6} } &
\colhead{\% \tablenotemark{7} }  & \colhead{uniform?\tablenotemark{8}} %
  }   
\startdata
% Cluster    R   fld      Nexp  Q1   Q2   Q3   Q4  In   Out  Ncand TotObs  TotPerc  Even?
% Name  &      & ($h_{75}^{-1}$Mpc)&    &     &    &    &    &    &    &     &     &      &     \nl \hline
Abell   98 & 3 & 3.0x5.1 &  8 &  57 & 56 & 64 & 73 & 62 & 59 & 253 & 152 & 60.0 & yes \nl
Abell  160 & 0 & 3.7x3.5 & 13 &  69 & 73 & 54 & 68 & 94 & 54 & 337 & 224 & 66.5 & marg,rad \nl
Abell  690 & 1 & 3.6x3.6 & 19 &  81 & 79 & 66 & 83 & 74 & 79 & 225 & 172 & 76.4 & yes \nl
Abell 1446 & 2 & 3.0x3.0 &  4 &  43 & 42 & 47 & 38 & 34 & 50 & 191 &  81 & 42.4 & yes \nl
Abell 1684 & 0 & 2.6x2.6 &  5 &  78 & 67 & 88 & 83 & 58 & 90 &  85 &  66 & 77.7 & marg,rad \nl
Cl1313+073 &-0 & 3.1x3.1 &  8 &  62 & 52 & 52 & 62 & 69 & 52 & 190 & 109 & 57.4 & yes \nl
% Abell 1569 & 0 & 4.2x4.2 &    &  83 & 90 & 67 & 67 & 73 & 79 &  70 &  53 & 75.7 & yes \nl
Cl1919+479 &-0 & 3.0x3.0 & 13 &  72 & 60 & 88 & 89 & 64 & 86 & 337 & 232 & 76.3 & yes \nl
Abell 2214 & 0 & 4.3x4.3 &  4 &  33 & 50 & 78 & 59 & 33 & 67 & 140 &  73 & 52.1 & marg,rad \nl
Abell 2220 & 0 & 6.3x6.3 &  3 &  81 & 100& 58 & 65 & 97 & 65 &  95 &  71 & 74.7 & marg \nl
Abell 2462 & 0 & 5.2x5.2 &  8 &  38 & 30 & 31 & 41 & 54 & 19 & 444 & 153 & 34.5 & No,rad \nl
Abell 2634 & 1 & 3.8x4.3 & 33 &  74 & 74 & 66 & 56 & 90 & 57 & 536 & 368 & 68.7 & No,rad 
\tablenotetext{1}{Abell Richness count.}
\tablenotetext{2}{Search field dimensions in $h_{75}^{-1}$Mpc. (The search field
was rectangular for A98 because of its bimodal appearance in X-rays.)}
\tablenotetext{3}{Number of 1 hour exposures taken with MX.}
\tablenotetext{4}{Subregion designation: Q1=upper right quadrant, 
Q2=upper left, Q3=lower left, Q4=lower right, In=inside circle of
diameter=1/2 of the field height, Out=outside of this circle.}
\tablenotetext{5}{Number of candidate galaxies in MX catalog.}
\tablenotetext{6}{Number of sampled candidates, i.e., those with at least 1 
spectrum.}
\tablenotetext{7}{Percentage of candidates sampled in the entire search field.}
\tablenotetext{8}{Estimate of how evenly the subregions are sampled. No= the
sampling percentages are significantly different in some subregions (Poisson
statistics), marg= the sampling is only marginally uneven, yes= the sampling
is fair and even, rad=the In and Out percentages are significantly different.}
% \tablrefs{   }
% \tablecomments{ }
% Note: the A160 Nobs includes 2 from P. Gomez's, 1995 run.
\enddata
\label{spatial}
\end{deluxetable}


